Investigating grammatical abstraction in language models using few-shot learning of novel noun gender

Humans can learn a new word and infer its grammatical properties from very few examples. They have an abstract notion of linguistic properties like grammatical gender and agreement rules that can be applied to novel syntactic contexts and words. Drawing inspiration from psycholinguistics, we conduct a noun learning experiment to assess whether an LSTM and a decoder-only transformer can achieve human-like abstraction of grammatical gender in French. Language models were tasked with learning the gender of a novel noun embedding from a few examples in one grammatical agreement context and predicting agreement in another, unseen context. We find that both language models effectively generalise novel noun gender from one to two learning examples and apply the learnt gender across agreement contexts, albeit with a bias for the masculine gender category. Importantly, the few-shot updates were only applied to the embedding layers, demonstrating that models encode sufficient gender information within the word embedding space. While the generalisation behaviour of models suggests that they represent grammatical gender as an abstract category, like humans, further work is needed to explore the details of how exactly this is implemented. For a comparative perspective with human behaviour, we conducted an analogous one-shot novel noun gender learning experiment, which revealed that native French speakers, like language models, also exhibited a masculine gender bias and are not excellent one-shot learners either.

==> notes <==
For example, humans can infer the gender of a new noun in French by association with the masculine article `le\textsubscript{m} wug' instead of the feminine alternative `la\textsubscript{f}. They can then easily perform grammatical agreement in various other unseen contexts such as choosing the corresponding masculine adjective in a sentence: `le\textsubscript{m} wug est vert\textsubscript{m}' [`the wug is green'] instead of the feminine alternative `verte\textsubscript{f}'. 

Importantly, this study contributes to answering whether models genuinely acquire abstract grammatical knowledge through such mechanisms or merely learn statistical patterns associated with abstract rules. 

The emergence of biases and difference in learning dynamics calls for further evaluation into the underlying mechanisms of such generalisations to determine if they are truly abstract. 

still leaves the question of whether model representations of gender are truly abstract unanswered.

and whether this is in line with psycholinguistic theories of generalisation as well as behavioural evidence.

The emergence of gender bias and difference in learning mechanisms across models provides possible ways of representing grammatical properties, which may be different to human linguistic theories and reflect actual human behaviour.

These sparse networks observed in LSTMs do contrast with human language processing which relies on a much more distributed system \citep{Bates2002LanguageBrain,Fedorenko2020LackNetwork}. Nevertheless, this type of mechanistic exploration of language models together with an understanding of how grammatical properties are represented and generalised from embeddings, contributes to theories about processing of syntactic structure and abstraction by humans.

For gender,the best candidate seems to be‘kind,’ which is too vague, however,to distinguish genders from other classes of words. More specifically,there are two major semantic domains often mentioned in relation to gender:sex and animacy(Corbett,2011b).

Animacy (antonym: inanimacy) is a grammatical and semantic feature, existing in some languages, expressing how sentient or alive the referent of a noun is. Widely expressed, animacy is one of the most elementary principles in languages around the globe and is a distinction acquired as early as six months of age.

Results
Another possibility that may contribute to slowing down learning is that the representation of the novel noun becomes semantically implausible with more training examples, as the learning sentences were not designed to be semantically consistent. However, this cannot explain why only feminine learning trials are affected negatively and only in specific conditions.

The human behavioural results, in comparison with model variances in error patterns and learning mechanisms, highlights the interplay of various factors influencing linguistic processing and gender generalisation including syntax, related words, semantics, in humans morphology and phonetics, and also learnt biases

The representation of grammatical gender and gender agreement rules across models provides alternative ways of representing grammatical properties that mimic human performance yet differ in how gender is devised by linguistic theories.

In a related analysis, for a given novel noun, we measured the weight change along the gender-direction. We define the gender-direction as the vector difference of two original noun embeddings were used in the composition of the novel noun. We confirm that projections of the nouns' weight change along the gender-axis was consistently negative (feminine), positive (masculine), or near zero in a gender-neutral control case according to the learning examples. 
\textcolor{purple}{Our few-shot word-learning and testing paradigm can be extended to include extensive tests of grammatical gender agreement, and more complex linguistic constructions such as nested-dependencies and testing agreement across attractor nouns with contradicting number or gender \citep{Marvin2018TargetedModels}. This framework can also be used to test grammatical abstraction in multilingual LSTMs, other Transformer architectures and the transfer of grammatical representations learnt across languages \citep{Gonen2022AnalyzingModels,Mueller2020Cross-LinguisticModels} and model architectures.}



\begin{table*}[h]
\begin{center} 
\renewcommand{\arraystretch}{1.3}
\tabcolsep=0.45cm
\small
\begin{tabular}{lll}
\hline
\vspace{0.2cm} 
&\raisebox{-0.4\normalbaselineskip}{\textbf{Learning example}} & \raisebox{-0.4\normalbaselineskip}{\textbf{Test (3 distractors)}}\\
\hline
\textbf{A}& article-noun & noun-adjective \\\hline
&j'ai vu \textbf{le}\textsubscript{m}/\textbf{la}\textsubscript{f} \underline{\textbf{noun}} &
je ne vois pas de \underline{\textbf{noun}} qui est très \textbf{vert}\textsubscript{m}/\textbf{verte}\textsubscript{f} \\\vspace{0.3cm} 
&{\small (I saw \textbf{the}\textsubscript{m/f} \underline{\textbf{noun}})} &
{(I don't see a \underline{\textbf{noun}} that is very \textbf{green}\textsubscript{m/f})}\\
\hline
\textbf{B}& article-noun & noun-participle \\\hline
&j'ai vu \textbf{le}\textsubscript{m}/\textbf{la}\textsubscript{f} \underline{\textbf{noun}} &
je ne vois pas de \underline{\textbf{noun}} plus ou moins \textbf{fixé}\textsubscript{m}/\textbf{fixée}\textsubscript{f}  \\\vspace{0.3cm} 
&{(I saw \textbf{the}\textsubscript{m/f} \underline{\textbf{noun}})} & 
{(I don't see a more or less \textbf{fixed}\textsubscript{m/f} \underline{\textbf{noun}})}\\
\hline
\textbf{C}& noun-adjective & noun-lequel/laquelle \\\hline
&je vois l'\underline{\textbf{noun}} \textbf{noir}\textsubscript{m}/\textbf{noire}\textsubscript{f} & 
je vois l'\underline{\textbf{noun}} très marron sur \textbf{lequel}\textsubscript{m}/\textbf{laquelle}\textsubscript{f}  \\\vspace{0.3cm}
&{(I see the \textbf{black}\textsubscript{m/f} \underline{\textbf{noun}})} &
{(I see the very brown \underline{\textbf{noun}} on \textbf{which}\textsubscript{m/f})} \\
\hline
\textbf{D}& noun-participle & noun-lequel/laquelle \\\hline
&je vois l'\underline{\textbf{noun}} \textbf{brisé}\textsubscript{m}/\textbf{brisée}\textsubscript{f} & 
je vois l'\underline{\textbf{noun}} très marron sur \textbf{lequel}\textsubscript{m}/\textbf{laquelle}\textsubscript{f} \\\vspace{0.3cm}
&{(I see the \textbf{broken}\textsubscript{m/f} \underline{\textbf{noun}})} &
{(I see the very brown \underline{\textbf{noun}} on \textbf{which}\textsubscript{m/f})} \\
\hline
\end{tabular}
\caption{Example sentences with three interfering words for few-shot learning and testing phases. We used tests with up to six distractors between noun and target; examples show tests three interfering words. The novel noun is underlined, the target word is bolded, and subscripts (f: feminine, m: masculine) indicate gender.}
\label{tab:tests_long}
\end{center}
\end{table*}
